An Energy Management System Approach for Power System Cyber-Physical Resilience

Power systems are large scale cyber-physical critical infrastructure that form the basis of modern society. The reliability and resilience of the grid is dependent on the correct functioning of related subsystems, including computing, communications, and control. The integration is widespread and has a profound impact on the operation, reliability, and efficiency of the grid. Technologies comprising these infrastructure can expose new sources of threats. Mapping these threats to their grid resilience impacts to stop them early requires a timely and detailed view of the entire cyber-physical system. Grid resilience must therefore be seen and addressed as a cyber-physical systems problem. This short position paper presents several key preliminaries, supported with evidence from experience, to enable cyber-physical situational awareness and intrusion response through a cyber-physical energy management system.

==> Implementation.tex <==
\section{Implementation}\label{sec:implementation}
%% kate 5/14/14 a lot of this is repeated, can be condensed 

\name system is composed of modules that distribute the work along logical lines and support the implementation of the contingency analysis algorithms as a real-world tool.  The functions described have been implemented in real software. While this framework uses information about the current state of the system, it does not interfere with or introduce delays into real-time data streams from sensors or command stream from operators.
%%Luis 5/14/14, 2:08 PM I agree with Kate. The Core analysis overview section should start here after the above intro sentence and merge the following 4 paragraphs with the current core analysis overview section  

\subsection{Core Analysis Overview}
The core analysis and model generation blocks of Figure \ref{fig:functionalBlocks} are implemented in a modified version of Zabbix ~\cite{ZABBIX}. Zabbix is a commonly used open source monitoring software package for enterprise networks which can be used to monitor the performance and availability of hosts and network hardware within a network.  For our implementation, the Zabbix code has been modified to manage the entire \name system, including the data input and output, as well as the functional blocks.  One of the components Zabbix manages is an interface to the power systems analysis block of Figure \ref{fig:functionalBlocks}, carried out by a modified version of PowerWorld \cite{simulator2005powerworld}.

In \name, Zabbix acts as a server and performs the initial contingency analysis based on both the input model as well as the performance indices retrieved from PowerWorld. The input model for the contingency analysis is generated using the NP-View tool~\cite{NPView}, which performs a comprehensive security analysis of the access policy rules and produces the network connectivity matrix according to the control network topology~\cite{SOCCA2014}. Zabbix is also configured to respond to detected failures (e.g., a network intrusion or failure of a critical process on a monitored agent) by triggering the analysis to be updated.  During the normal course of operation, this includes updating the security state by asking the power system analysis block to calculate a new security index for the predicted next most likely outages. Thus, Zabbix keeps track of the current POMDP state of the system and updates the PowerWorld interface accordingly. 

Updating the security state requires knowledge about the location of the host in the network, what other hosts are reachable from the compromised hosts, what vulnerabilities exist on those hosts, and the physical impacts of the compromised hosts on the power system. To that end, \name uses a threat model, power system physical model and simulation capability, a cyber network topology model along with the inter-host accessibilities according to the global firewall rulesets, as well as the cyber physical mapping that contains the points of cyber-physical interconnection. The network model allows us to see where in the network misbehaving host is located. The cyber-physical mapping lets us evaluate the potential physical consequences using the power system analysis software.  The threat model enables \name to assign transition probabilities between the security states.

The time scales at which information must be exchanged determine what data transmission methods are appropriate.  Our \name implementations use sockets for fast and frequent data exchange and files for less frequent data exchange.  The power system side is frequently being asked to gauge the impact of a contingency, so the communications must be relatively fast.  Thus, the Zabbix-PowerWorld communication uses network sockets.  The threat model, power system model, and cyber network model are parsed from files.

The standard PowerWorld Simulator software package has been heavily modified to allow it to accept and send data over a TCP socket. The original use of this feature was for an operator training simulator \cite{PWTrainer},
%\footnote{Available at \url{http://www.powerworld.com/products/trainer/overview}}
where multiple operators interact with the same case.  The modifications for the present application allow the software to 1) accept a case sent from a server, 2) accept commands to change data in the model, and 3) return data about the model to the server.  

The protocol implementation follows the sequence outlined in Fig. \ref{fig:ZabbixPW}.  Zabbix acts as the server, listening for connections.  The modified PowerWorld code connects to the listening Zabbix process and waits for commands.  The connection is maintained throughout the process.  Once connected, PowerWorld will receive, interpret, and reply to the Zabbix commands.  Zabbix is able to formulate the commands and interpret PowerWorld's responses.  The payload of a sockets message contains data that is required for the command to be successfully executed.  It can be as large as the power system case file, or it may simply be an identifier of a field and a value to retrieve. 

% kate 1/12/15 the paragraph that was already here already addressed the new reviewer comments, I thought, but trying to make it more explicit now...
PowerWorld and Zabbix must communicate using exactly the same message protocol and data formats.  The payload is a byte stream, and PowerWorld and Zabbix must both know how to interpret it.  The framework can be adapted to be used with other security event management systems and to integrate with other energy management systems.  

% kate 1/12/15 previous text:
%The Zabbix and PowerWorld implementation presented here provides just one practical example. There are many monitoring and event management systems in use including ArcSight, Synamtec, and Splunk.  Similarly, utilities use a variety of energy management systems including those by Alstom, ABB, and OSI. In theory, one could realize a CPMA framework using any combination of the commonly used event manager and energy management systems.  

% kate 1/12/15 from prev. response doc, reworded:
The implementation described here uses our own code, the modified source code of PowerWorld and Zabbix, and the software tool NP-View.  This is just one of the many possible ways to implement the CPMA system. Zabbix was chosen as the cyber monitoring system because it is an open source solution commonly used in enterprise network monitoring. PowerWorld was chosen because PowerWorld is widely used in the power industry and its source code could be modified directly by the authors for this work. 
NP-View has been originally developed at the University of Illinois at Urbana-Champaign to support the power industry to determine control network topology and security.  We chose to use NP-View to parse and analyze the network topology and architectural security measures in the network because it made it easy for us to obtain the information we needed. Any means of obtaining the cyber network topology may be used, although in all cases the topology would have to be converted to a format CPMA can use. 
There are many different Security Information and Event Management (SIEM) systems in use including ArcSight, Symantec, and Splunk. Any of the available SIEM systems could potentially be adapted to replace Zabbix in our implementation. Similarly, there are a variety of power system analysis tools in use including those by Alstom, ABB, and OSI. While Zabbix and PowerWorld are used here, the algorithms and protocols are agnostic to specific implementations and can be adapted to different platforms and different programs.



%RBOBBA 09/12/14 ---The following are the core set of messages and commands used to achieve these interactions. 

\subsection{Server and Client Messages}
A prefix is attached to Zabbix-PowerWorld messages to identify the sending host.  Messages sent from the server begin with \textbf{tsm}, while those from the client begin with \textbf{tcm}.  The relevant messages that allow us to implement the client-server communication are described below.  The Zabbix process is the server, and PowerWorld is the client.

\begin{itemize}

\item \textbf{tsmSendCase.} The server sends a message that includes a new power system model.

\item \textbf{tsmSetData.}  The server tells the client to set the specified fields to the specified values for the specified objects.  The PowerWorld client will set the specified fields and automatically solve the power flow upon receipt of the message.
	
\item \textbf{tsmGetClientState.} The server requests the present values of the specified fields for the specified objects in the case from the client.  The PowerWorld client retrieves the values of the specified fields and returns them using a tcmSendData command.

\item \textbf{tcmSendData.} The client sends specific information about the system back to the server in response to a tsmGetClientState command.


\end{itemize}


\subsection{Zabbix-PowerWorld Communication Protocol}

\begin{figure}
\centering
%\includegraphics[scale=1]{ZabbixPW.png}
\includegraphics[scale=.75]{zabbixpwfixed.pdf}
\vspace{-0.2in}
\caption{Zabbix-PowerWorld communication}
\label{fig:ZabbixPW}
% kate 9/13/14 the below was making the figure caption overwrite other text..
%\vspace{-0.2in}
\end{figure}


%%% kate 5/14/14 this section could be completely merged with subsection above, keeping the sequence of the protocol and splicing in the examples from the above subsection
The communications are illustrated in Fig.~\ref{fig:ZabbixPW}, starting with the initial connection.  Once the connection is established, it is kept open. When a case is ready for analysis, it is sent to the PowerWorld client, where it is immediately opened and placed in memory. The program below shows the code to send the case.  This command is sent at the start of the analysis and periodically as new state estimates become available.  
%When this command is sent, the receiving client immediately opens the case, replacing the case in memory.
\begin{program}
\small
\label{ex:sendcase}
\begin{verbatim}
SendFile( std::string("case.pwb"), tsmSendCase, 
     true, connectedList[c]->socket());
\end{verbatim}
\caption{Example of sending new case}
\vspace{-0.1in}
\end{program}



Then, \name uses tsmGetClientState and tcmSendData to retrieve data for all of the lines in the case.  It is critical for Zabbix to know the correct labels or names of the lines in order to manage cyber-power interconnections as well as line outages.  The program below shows the code to open one of the lines, identified by its label.

%************** OPEN LINE BY LABEL **********
\begin{program}
\small
\label{ex:getlines}
\begin{verbatim}
objectID = "BRANCH 'Capital City$BRK$4647'";
FieldID  = "LineStatus";
Value    = "Open";
SendSetDataMessage(tsmSetData, connectedList
     [c]->socket(), ObjectID, FieldID, Value); 
\end{verbatim}
\caption{Example of sending command to open line}
\vspace{-0.1in}
\end{program}

%************** GET PERFORMANCE INDEX ****************

\begin{program}                              
\small
\label{ex:getpi}
\begin{verbatim}
objIDs.add("PWCaseInformation");
fldIDs.add("OverloadRank");
SendGetData(tsmGetClientState, true, 
     connectedList[c]->socket(), objIDs, 
     fldIDs, 1 ); 
\end{verbatim}
\caption{Example of getting performance index}
\vspace{-0.1in}
\end{program}


During the contingency analysis, the Zabbix server will be sending requests to the PowerWorld Client to evaluate the effects of an outage in order to populate the security states.  This is shown as  ``Build or update POMDP" in Fig.~\ref{fig:ZabbixPW}.  The commands are used to apply an outage and request the security metric.

The program above shows the code that returns the performance index that is used to evaluate the severity of potential outages. This command is sent by the Zabbix server.


The tsmSetData command can also be used for visualization purposes.  There are several custom fields in the PowerWorld client that allow users to specify data stored with the objects in the model.  For example, a custom floating point field can be used to store post-contingency flows with each line.  Setting these fields in conjunction with utilizing other built-in features of PowerWorld allows users to create customized one-line diagrams and results displays. % including highlighted objects and text fields.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% end matt's text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Analysis Results}

\begin{figure}
\centering
\includegraphics[width=.45\textwidth]{size-crop.pdf}
\vspace{-0.1in}
\caption{Automatically Generated Model Size}
\label{fig:size}
\vspace{-0.1in}
\end{figure}

For the proposed framework to be practical in real-world settings, it is crucial to be efficient. In our experimental evaluation, we measured how large the generated models get. Results are shown in Figure \ref{fig:size}. We have employed mathematical finite look-ahead technique to produce models partially based on the system's current security state. The figure shows the size of the generated model given the state exploration depth starting from the current state. According to our experiments, the depth of 4 gives sufficiently accurate results in practical settings; however, for completeness of the results, we have included the model sizes up to the depth of 6 in Figure \ref{fig:size}. 

\begin{figure}
\centering
\includegraphics[width=.45\textwidth]{time-requirement-crop.pdf}
\vspace{-0.1in}
\caption{Analysis Time Requirement}
\label{fig:time}
\vspace{-0.1in}
\end{figure}

The size of the generated models represent the number of states in the produced Markovian decision processes for the control center; however, the time required to analyze those models may not be linearly dependent on the number of states, because the state transitions within the generated models play a key role in the contingency analysis's time requirement. Figure \ref{fig:time} shows how long \name requires to complete its analysis. As shown in the figure, the time required to complete the analysis in \name for a sufficiently accurate model (with state exploration depth of 4) is always below 1 second. This is promising for practical deployment of \name. 

\begin{figure}
\centering
\includegraphics[width=.47\textwidth]{robustness-crop.pdf}
\vspace{-0.1in}
\caption{Sensitivity Analysis of Contingency Rankings}
\label{fig:robustness}
\vspace{-0.1in}
\end{figure}

To further evaluate \name regarding its real-world deployability, we measured the robustness of its contingency ranking results against inaccuracies in the input data. In particular, the accuracy of the output contingency rankings by \name is a function of the state transition probabilities within the generated Markov decision process models. The state transition probabilities which represent the success rate given that their corresponding malicious actions are taken by adversarial parties are subjective measures. As such there is some uncertainty associated with these values. To be practical, \name will have to tolerate uncertainty in these state transition  probabilities. Figure \ref{fig:robustness} shows the results of our experiments. The horizontal axis shows the level of deviation (inaccuracy) in the input probability values, and the vertical axis represents the standard deviation of ranking position of top N (between 3 and 100) contingencies. This deviation is a measure of how much a particular contingency's ranking changes as the input probability values deviate from their true values (horizontal axis). As evident from the figure, contingency ranking results provided by \name demonstrate robustness against uncertainty. In particular, the standard deviation stays low even when the probability values for state transitions involve inaccuracies of up to 0.25. 



==> ModelGeneration.tex <==
\section{Model Generation}\label{sec:modelgen}
% kate 5/13/14 we might want to merge this section and the SOCCA section some or just make sure they read well together

Modeling cyber-physical infrastructures concisely is challenging.  Accurate hybrid automata models can impact scalability significantly, and traditional discrete modeling techniques do not consider the physical components. Instead, \name makes use of an extended discrete state-based model, i.e. a partially observable Markov decision processes (POMDP), that captures sufficient information about the physical system for analyses without causing practical scalability issues. The POMDP enables \name to model the underlying cyber-physical infrastructure and estimate its current probabilistic state considering uncertainties in sensor measurements. 

%Generally,  
Every cyber-physical attack path consists of an escalating series of vulnerability exploitations by the adversary. Initially, the adversary does not have access to the network, but eventually achieves the privilege required to reach his or her attack goals, e.g., causing a power transmission line outage by opening a relay. States in the POMDP capture only the necessary information about the system for our later contingency analyses. Each state is represented as a bit vector where each bit indicates the secure or compromised status of a computing device, e.g., a control center host. Therefore, the initial state is $\varnothing$, in which the attacker does not yet have any privileges over the smart grid network. Each adversarial state transition represents a privilege escalation which is achieved through a vulnerability exploitation. Therefore, any path on the POMDP graph represents an attack path in the power network.

More specifically, each security attack is in a finite set of security states $S$ that cover all of the system's possible security conditions. The system is in one of the security states $s$ at each time instant. From the system's current state, the attacker chooses and takes a malicious action $a \in A$ admissible in $s$, \ie an exploitation that is feasible,  which leads to a transition to $s'$. At each transition, the attacker may receive a reward according to a specific reward function for that type of attacker, e.g., a hacker seeking financial gain.
The reward function value is the amount of his or her interest in the corresponding state. 

Formally, a discrete Markovian decision process $\Gamma$ is defined as a tuple $(S, A, R(.), P, \gamma)$ where $S$ is the security state space, endowed with the discrete topology. At every time point, the system state is represented as a probability distribution over the state space due to the false positive/negative rates of the IDS alerts. $A$ is the set of adversarial actions. At every $s \in S$, $A(s) \subset A$ is the set of admissible actions.
%at state $s$. 
The measurable function $R: S \to [0,1]$ is the adversary-driven reward function calculated for each state based on the power system performance index value in that state \cite{chiang1995toward}. For example, if a relay is connected to a circuit breaker, and that relay is compromised, we assume the consequence is measured by the severity of the electrical system impact caused by opening that breaker. 
%Additionally, in the cyber-side exploitation steps of the attack, 
The reward is also a function of \textit{ease of attack}, i.e., how easy the target vulnerability is to exploit. $P$ denotes the transition probability function; that is, if the present state of the system is $s$, taking an action $a$ results in a state transition to state $s'$ with probability $P(s'|s, a)$. 
%An immediate reward $R(s')$, i.e., adversary-driven reward value of the state $s'$. 
$\gamma$ is the discount factor and is normalized, i.e., $0 < \gamma < 1$.


The smart grid network's access control policies, such as firewall rulesets, are composed of rules about sources (IP and port addresses) that are either allowed or not allowed to reach a destination. \name parses the rulesets and creates a binary network connectivity matrix that is a Cartesian product of host systems. The $[i,j]$ entry of the matrix takes on a true value if traffic from host $h_i$ to host $h_j$ is allowed, and a false value if it is not allowed. The connectivity matrix always includes an Internet node representing a group of hosts outside of the network, where attackers are assumed to initially reside. \name generates a comprehensive POMDP model of the smart grid network that represents all \emph{possible} attack paths. The generated POMDP by design address all system vulnerabilities and could partially account for previously unknown exploitations by having a small probability of transition even on paths where no known vulnerabilities exist.

Generation of Markov decision processes (attack graphs) based on the automated extraction and analysis of network firewall rules
% kate 9/13/14 not necessary, stated elsewhere
%\footnote{We make use of NP-View software to parse and analyze the network topology and architectural security measures in the network.}
% kate 9/13/14 a bit apprehensive about saying "all" attack paths; it's really just all attack paths that are captured by the NP-View firewall rules
ensures comprehensive coverage of possible attack paths.  Based on the firewall rules, our tools pessimistically consider all the computers that are accessible from a particular host system to be vulnerable, and hence compromisable, by the adversaries. Consequently, the generated attack graphs incorporate every feasible single or multi-step attack vector through the control center network that could potentially cause a physical power system consequence, e.g., a malicious circuit breaker trip. 

==> OverviewFramework.tex <==
\section{Cyber-Physical Resilience Framework}






%\begin{itemize}
%\item 

%%% Functional blocks %%%

%\begin{itemize}
%\item 










==> RelatedWork.tex <==
\section{Related Work}

Over the last few years, design and analysis of cyber-physical systems have received considerable attention in the research community.  There has been a lot of work proposing to model and analyze cyber-physical systems in general and in power grids specifically. We review works closely related to our approach and discuss their merits. 

In~\cite{lee2008cyber}, an early paper on the topic, Lee discussed design challenges for cyber-physical systems and argued that existing abstractions and modeling techniques are inadequate for cyber-physical system design. Specifically, he contended that while there are modeling solutions for discrete cyber networks as well as continuous physical plants, the current tools do not sufficiently account for the cyber-physical interconnections and more accurate algorithms and tools are needed in the field. Derler \etal \cite{derler2012modeling} discussed the challenges in modeling cyber-physical platforms. In particular, the authors named intrinsic heterogeneity, concurrency, and sensitivity to timing as the challenging factors. More specific to energy, Ilic \etal \cite{IlicXKM08} proposed cyber-physical models of generation and load components and their interconnection through the electrical network. Their work was focused on load modeling and did not consider the cyber network. Palensky \etal \cite{PalenskyWE14} discussed the challenges associated with continuous-time and discrete-time cyber-physical models of energy systems and compared the scalability of these two approaches.

Security and reliability of the cyber-physical energy infrastructures has also received considerable attention (\eg  \cite{CardenasAS08,LiuFKZB11,Garcia12,Zonouz12,SOCCA2014}). A switched systems view of the power grid is used by both \cite{LiuFKZB11,Garcia12}. Liu \etal \cite{LiuFKZB11} used it to model coordinated cyber-physical attacks, while Dominguez-Garcia \cite{Garcia12} used it for reliability modeling. Challenges facing secure control and survivability of cyber-physical systems were discussed in \cite{CardenasAS08}. They suggest as missing an ability to estimate the state of the cyber network along with the state of the physical system and an ability to use that information in improving the physical system's performance. In \cite{Zonouz12}, Zonouz \etal proposed a framework that leverages estimates of security state of the cyber infrastructure to improve electrical system state estimation. In \cite{zonouz2009rre, zonouz2012elimet}, security-oriented techniques for effective steady state cyber-physical abstraction using stochastic control algorithms are introduced. They also discussed how such models could be used for automated decision-making for optimal response actions against adversaries who target safety-critical infrastructures. However, \cite{zonouz2009rre, zonouz2012elimet} concentrated mostly on the computational assets and did not consider power system dynamics in details in their analyses. 

This work builds upon cyber-physical power systems analysis of SOCCA~\cite{SOCCA2014} by using a POMDP to improve the analysis of cyber-induced contingencies, and  by including an estimate of the security state. Chen \etal \cite{Chen2013}, proposed a workflow based security assessment framework and demonstrated its use using the case of Advanced Metering Infrastructure. Their work is limited to the assessment of the cyber-infrastructure and does not take the electrical infrastructure into account. However, their work can be leveraged to improve the scalability of our threat modeling and is complementary to our framework. 



%This work is also focused on how the results of the anlaysis can be applied to provide the greatest benefit to utilities.  

%SOCCA focuses on the fundametal theory showing that combined cyber-physical analysis co-utilizing cyber side and power side data can be performed to achieve results indicating, in summary, which cyber contingencies are most important for an organization to defend against in order to thwart attacks with the greatest risk, where risk is measured by ease of implementation combined with the scale and range, or quantity, of impact.

%This work builds upon SOCCA by examining exactly what is needed for such a model to succeed and to be beneficial to utilities. We focus on what information can be obtained from a combined cyber-physical model and its analysis, i.e., how the analysis can be applied to provide the greatest benefit to utilities.


\begin{comment} %backup - RBB
\textbf{Cyber-physical system modeling.} Lee \cite{lee2008cyber} introduced the problem for the first time and argued whether the existing modeling techniques are adequate for cyber-physical system modeling and analysis purposes. He discussed that while there are modeling solutions for discrete cyber networks as well as continuous physical plants, the current tools do not sufficiently account for the cyber-physical interconnections and more accurate algorithms and tools are needed in the field. Derler et al. \cite{derler2012modeling} discussed the challenges in modeling cyber-physical platforms. In particular, the authors named intrinsic heterogeneity, concurrency, and sensitivity to timing of CPSs as the challenging factors. Zonouz et al. \cite{zonouz2012scpse, zonouz2009rre, zonouz2012elimet} introduced a security-oriented technique for effective steady state cyber-physical abstraction using stochastic control algorithms and focusing on scalability. They also discussed how such models could be used for automated decision-making upon optimal response actions against adversaries who target safety-critical infrastructures.
\end{comment}


\begin{comment} %not very relevant - RBB
\textbf{Hybrid system analysis and control.} Typical properties studied theoretically for secure and safe hybrid dynamical systems include the nature of asymptotic equilibria \cite{aastrom2012introduction}, stability \cite{kimbark1995power}, reachability \cite{aastrom2011computer}, formal verification \cite{chutinan2003computational} and model checking \cite{henzinger1997hytech}, the effect of parameter changes (sensitivity) analysis \cite{dullerud2000course}. On the security side, there have been several past attempts to design automated security assessment techniques \cite{zonouz2013seclius} that could adaptively infer configuration and communication patterns of any specific networked infrastructure. Most importantly, data-tainting and information tracking analysis techniques have been proposed for malware detection \cite{yin2007panorama}, for offline forensic analysis using backtracking \cite{king2005backtracking, jiang2006provenance} or forward-tracking techniques \cite{zhu2003design}, and for online damage situational awareness \cite{liu2010cross}. In \cite{liu2010cross}, information flow is tracked across multiple layers, namely at the instruction level and at the OS process level. Such dynamic information tracking solutions often require high computational resources, which makes most of them infeasible to deploy in real-world complex settings.
\end{comment}



==> SOCCA.tex <==
\section{Cyber-Physical Security Analysis}\label{sec:socca}

%Cyber-physical security analysis or SOCCA is used to determine outages that, due to cyber connectivity, have a greater likliehood of occuring.  

The core cyber-physical security analysis algorithm used in the proposed framework builds on top of SOCCA~\cite{SOCCA2014} which is an \textit{offline} power grid analysis tool. However, for this work on \textit{online} security state estimation and cyber-physical contingency analysis, we use the POMDP that captures potential paths an adversary could take through a network to cause cyber-physical events that we call contingencies. The partial observability is a crucial feature, as during the online analysis, it is infeasible to exactly determine the current state of the system, given the noise and false positive/negative rates of the power and cyber security sensor reports. 


Starting from the POMDP's initial state $\varnothing$, an adversary could then reach a state where it is possible to send a command resulting in a physical consequence. As discussed above, the reward to the adversary of taking action $a$ from state $s$ is $R(s,a)$.  
%%% REWARD FUNCTION %%%
The reward function is the following,
\begin{equation}
R(b,a)  =  \sum_{s \in S} b(s) \cdot \sum_{s' \in S} P(s'|s,a)[\Delta F(s,s') + I(s')]
\end{equation}
where $b$ is the current \textit{belief} state of the system, i.e., a probability distribution over the state space of POMDP. Clearly at each time instance, we have $\sum_{s \in S} b(s) = 1$. $F(s)$ is a performance index defined in each state.  
%%%% PERFORMANCE INDEX %%%%
The performance index is computed using the following equation, which measures the severity of a transmission line outage based on the subsequent line overload(s):
\begin{equation}\label{eq:performanceindex}
F(s) =  \sum_{l \in L}  \big[ \max\{\frac{f_s(l)}{f^{MAX}(l)}-1,0 \} \big] ^2.
\end{equation}
Here, $L$ is the set of all lines, $f_s(l)$ denotes flow on line $l$ in state $s$, and $f^{MAX}(l)$ denotes the maximum flow allowed on line $l$. 

%%% SECURITY INDEX %%%%
The POMDP's value function for each state is the cyber-physical security index $I(s)$, which is evaluated by solving the following dynamic programming equation:
\begin{equation}\label{eq:dynprog}
%I(s) = \max_{a \in A(s)} \{\gamma\cdot \sum_{s' \in S} P(s'|s,a)[\Delta F(s,s') + I(s')] \},
I(s) = \max_{a \in A(s)} \{\gamma\cdot R(s,a) \},
\end{equation}

The level of fitness to an adversary of a cyber attack step is represented by the transition probability $P(s'|s,a)$ and the physical impact $\Delta F(s,s') = F(s') - F(s)$.  
%The normalized discounting factor $\gamma$ represents the fact that a reward now is worth more than the same reward in the future. 

To evaluate the attack severity in each state, the framework deploys a full power system simulation. We evaluate the effect of each reachable switching action (a breaker opening) and solve the AC power flow equations using the iterative Newton-Raphson algorithm to calculate the line flows. This impact is incorporated into the severity metric in each POMDP state as in Equation \ref{eq:performanceindex}. Note that modeling variations are possible for the power systems analysis.  The appropriate method depends on the needs of the utility and the purpose of the analysis. 
%Could be more specific here
For example, an approximate DC model may be used, requiring only a non-iterative linear solution, but sacrificing accuracy \cite{dcpowerflowrevisited}. 


% kate 5/2/14 Re-write.  Idea is to talk about extensions/ broader applicability
%\subsection{Other security metrics}
It is noteworthy that it is also possible to expand this framework by extending the capabilities of the individual components.  For example, modeling a lighting strike that affects power lines as well as communications lines could be done if the power system model is able to simulate electromagnetic transients and the cyber system model contains the physical connections of the communications lines.  Also, it is possible to use this framework to evaluate the transient stability of the system due to a cyber compromise by adapting the modeling techniques.  While this is beyond the scope of our present work, the framework is extensible to other cyber-physical analysis applications.


%types of result information produced
  \vspace{-0.1in}
\subsection{Result Interpretation}
Our framework explores and analyzes potential cyber-physical contingencies according to the current probabilistic cyber-physical state estimate and provides a risk-based ranked list. In particular, for a scalable state space exploration, we make use of the maximum likelihood approximation algorithm, and first pick the state with the highest estimation probability according to the sensor measurements, i.e., $s^* = \arg\max_{s \in S} b(s)$. The analysis results are represented using a three-value tuple for each state $(ID, F, I)$.  The first value is an identifier.  This identifier corresponds to the specific set of hosts and devices that have been compromised in that state.  The second number is the performance index $F(s^*)$, i.e. the immediate physical consequence of being in that state.  The performance index is only non-zero for states that are connected to a device such as a relay that is capable of performing a physical action such as opening a breaker.  The third number is the security index $I(s^*)$, recursively evaluated for each state.  In interpreting the results, the security index represents the best choice from an adversarial perspective.  For example, in the below highly simplified POMDP of Figure~\ref{fig-statespace}, one can trace the graph by following the greatest values of $I(s^*)$ and determine the three most critical cyber-physical attack paths or contingencies.  These are tabulated in Table~\ref{tab:ranking}.

\begin{figure}[h]
\vspace{-0.1in}
  \centering
%  \includegraphics[width=0.3\textwidth]{statespace3.png} 
  \includegraphics[width=0.4\textwidth]{simplestatespace.pdf} 
  \caption{Sample state space graph}
  \label{fig-statespace}
  \vspace{-0.2in}
\end{figure}

\begin{table}[h]
\caption{Ranked Critical Paths}
\label{tab:ranking}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l l l l l l}
	\hline
	\hline   
	Path 1		 &  & & & &  \\
	\hline
	Step	&	$H_0$ $\rightarrow$ $H_1$	&	$H_1$ $\rightarrow$ $H_2$ & $H_2$ $\rightarrow$ $R_1$  & &  \\
    I(s)	&	0.817	&	2.58 	& 2.16 	   & &	\\
	\hline
    Path 2		 &  & & & & \\
    \hline
	Step	&	$H_0$ $\rightarrow$ $H_1$	&	$H_1$ $\rightarrow$ $H_3$ & $H_3$ $\rightarrow$ $R_2$ 	& &  \\
    I(s)	&	0.817	&	1.88 	& 2.4 		& &  \\            
    \hline
    Path 3		 &  & & & &\\
	\hline
 	Step	&	$H_0$ $\rightarrow$ $H_1$	&	$H_1$ $\rightarrow$ $H_3$ & $H_1$ $\rightarrow$ $H_2$ & $H_2$ $\rightarrow$ $R_1$ & $H_3$ $\rightarrow$ $R_2$\\
    I(s)	&	0.817	&	1.88 	& 4.06    &  6.83	& 13.77  \\
	\hline
	\hline
\end{tabular}
\vspace{-0.1in}
\end{table}
		

Figure \ref{fig:network-combined} shows these analysis results for a sample system.  The first path leads to the most critical line outage for the system in three steps.  The second path leads to the second most critical, also in three steps.  The third most critical path is the most interesting as it is also the most complex.  Here, the adversary's path leads into the control center first, but the adversary does \textit{not} yet open the breaker, which by itself would cause the second most severe contingency.  Then, the adversary backtracks and follows steps leading to opening a line in the Haverbrook substation, causing the most severe single contingency.  After that, the adversary proceeds to cause a double line outage and subsequent overloads approximately doubling in severity by taking out the second line, at the control center. He or she could have been dormant waiting for the Haverbrook outage and then knew that would be the most effective time to take out the line in the control center. This example shows how complex attacks can be identified, where these attacks potentially involve more than one action with a physical consequence. Our security analysis thus pinpoints weaknesses in the cyber infrastructure, that through compromise, can lead the system to be in an emergency state, from an operational reliability standpoint.  Notice that the highest ranked critical paths share several of the same elements and steps.  Thus, targeting protection efforts to the identified common elements can have a system-wide benefit.

It is reasonable to assume that such a double line outage would not normally be considered in a utility's standard planning procedures, as the lines are not geographically close or otherwise coupled.  While standard contingency selection methods may miss these contingencies, our framework predicts and flags them for further consideration.

% kate 5/2/14 - Could allude to what we mean by "further consideration" here -- talk about potential SCOPF type operation, like Rakesh's comments today.  I think that would be good.

\begin{figure*}[htp]
  \centering 
	\includegraphics[width=0.77\textwidth]{4panel4.pdf}
    \vspace{-0.2in}
  \caption{Cyber-originated threats: ranked critical paths for double line outage example}
\label{fig:network-combined}
\vspace{-0.2in}
\end{figure*}
 


%%%%%%%%%%% kate 5/5/14 below is from Q4 deliverable - I feel like we should mention this somewhere but I'm not sure where%%%%%%%%
\subsection{Real-World \name Stakeholders}
Given that the \name toolset undertakes cyber-physical analysis and spans both the cyber and power sides of the system, its corresponding stakeholders would be a combination of personnel from the operational technology and information technology divisions of a utility. Support engineers may be responsible for configuration and validation of the toolset while the operational personnel may be responsible for ongoing monitoring and response. Support engineers include both network engineers and SCADA/control engineers. Similarly, operators include both control room operators and network operations center (NOC) staff. To make \name accessible to the wide variety of roles, the analysis process is automated so that the end-users will ultimately see only the results applicable for their practical usage and do not have to manually sift through unnecessary low-level details of the system. 

% kate 9/9/14
Engaging these stakeholders is crucial for us to verify and validate the \name toolset.  We are presently working with several advisory members including utilities to ensure that our efforts target and solve real-world problems.  Part of this effort involves the evaluation of \name in a real utility system, which will be reported in future work.

\begin{comment}
%Stakeholders
\begin{itemize}
\item \textbf{SCADA Engineer}. The SCADA engineer has strong serial and dedicated circuit background and not as much switch packet networking understanding.  These engineers are used to hardware designs and troubleshooting as well as modem operations (dial-up, leased line, radio, Sat, Microwave). These might be most knowledgeable about communications between control center and substations.

\item \textbf{Substation Engineer}. The substation engineer has a wider experience with more technology and has bridged the gap between the network engineer and the SCADA engineer many times.  They have worked with serial control devices and bridge technology to merge legacy devices onto networks.  They have also worked with network devices at newer installations and connected into WAN technology with SONET, T1, MPLS, or other DSUs. These might be most knowledgeable about substation networks.

\item \textbf{Control Room Operator}. The control room operator is tasked with being the first eyes and ears on the system and with initiating incident response plans when the system starts to deviate from expected behavior.  They are watching the operations of the large assets on the power system to protect them from damage and to keep the staff safe and the system operational.  These operators want to have intuitive monitoring capabilities.
%and the system to automate or explain the correct response actions. 
\name tools should provide an intuitive interface to this audience. 

\item \textbf{Planning Engineer}. The planning engineer is responsible for long term planning for power system operations, as well as studies and analysis to facilitate such planning. Ensuring the system will meet operational reliability criteria is a primary focus.  Planning engineers might be the first contact points to demonstrate the \name technology and get buy-in. 


\item \textbf{Network Engineer}. The network engineer has a strong legacy network background. These engineers are used to having scripts to manage deployed network appliances and typically work to design the subnets, VLANs, and ACLs for each corporate network on the business system or control system.  They typically do not have control device experience. These might be the most knowledgeable about portions of the organization's cyber network topology.
%In the contect of \name, they will be providing needed information regarding the network topology.


\item \textbf{Network Operation Center (NOC) Operator}. The NOC Operators are similar to the Control Room Operators with one distinction; they monitor the communication infrastructure only and not the power system assets. These will be most knowledgeable about the network monitoring and IDS capabilities of the system, and the cyber security state estimation functionality in SOCCA is most relevant to this audience.

\end{itemize}
\end{comment}
%%%%%%%%%%%%%% end from Q4 deliverable %%%%%%%%%%%%



==> ScalableOnline.tex <==
\section{Real-World Aspects: Online Operation and Scalability}\label{sec:online}
\todo{0.75 p}


\subsection{Online updates and analysis adaptation}
%The framework in this paper extends the theoretical basics of the SOCCA concept in several key directions. [Enumerate these better, this should maybe occur earlier in the paper, or elsewhere??] 
This framework adapts SOCCA to a scalable, on-line analysis tool intended for a transmission operations environment.  The analysis is based on an estimate of the current cyber security state.  \textbf{[Security SE references, add more here]}  
(Note that ~\cite{SOCCA2014} examined only cases where the system's initial state was that of no attacker privilege and no contingency.)  
Details of the online analysis are given in Section [Implementation].  
Our objective with this implementation is to transform the SOCCA approach into a useful and practical tool for utilities. We follow this direction by integrating the power flow analysis with the security event management application at scale and in real-time.
 

- What you do to get the updates and update the current state and then the results, etc.

\subsection{Scalability}
- Firewall rules - assumptions about vulnerabilities and host connectivity?
- Finite horizon
% could even add Q4 example of the difference this makes in state space size

% If we only care about the top X (say 5) paths, do we even need to calculate the rest?  I wonder if there's a way not to have to calculate all of it?  For example, I know with like SVD, it's time intensive, but if you only care about the top X singular values, you can cut out a lot of the time and only calculate those and then stop.  I wonder if something similar can be done for MDPs? b/c much of the MDP we don't actually care about.  Just thinking..

%\subsection{Control center integration}
%- How the analysis can be applied to utilities/ potential utility benefits

%The integration into power flow analysis and security event management software as well as scalability enhancements for practical run-time considerations offers to transform the SOCCA fundamentals into useful utility tools.

==> ThreatModel.tex <==
\section{Cyber-Physical Threat Model}\label{sec:threat}

%How do we ensure trustworthy actionable data and applications?  
%The path to more trustworthy systems begins with a more in-depth understanding of the potential problems.  In order to design effective protection and detection mechanisms, we need the ability to characterize how attacks might look in a real power system and how they might be achieved from a practical standpoint. 

Threat modeling is a structured way of representing threats 
%\footnote{Used more broadly than to mean threat sources} 
against a system and is often an integral part of risk assessment or risk modeling for a system. 
%To shed light on the risk of a contingency caused through a cyber attack, which is the focus of our work, understanding the threats and the likely ways such threats could materialize is very important. 
In a cyber-physical system, along with threats to confidentiality, integrity, and availability of data, applications, and other cyber assets, it is also important to i) take into account the threats to integrity, availability, and safety of the physical system, and ii) to understand the interdependence between threats.
%For traditional IT systems threat modeling focuses on threats to confidentiality, integrity and availability of data, applications and other assets.

{\bf A sample attack vector.} Here we describe a sample cyber-originated multi-step attack vector that adversely impacts the underlying physical power system, with the potential to cause a catastrophic failure, e.g., an outage or brownout. The attackers are initially assumed to reside outside the power grid control center network. We do not consider physical attacks, e.g., breaking into the control center building. The attackers must penetrate the control center network through cyber vulnerability exploitations. However, not all of the control center computers are accessible from outside due to typical strict firewall rule settings. Often, publicly or semi-publicly accessible computers do exist, e.g., corporate web servers and third-party access points, that could be hacked into if their software contains vulnerabilities, e.g., buffer overflow. Once such accessible computers are compromised, the adversaries can use those systems as a stepping stone to further penetrate into other accessible systems in the network and get closer to control network and eventually to the power system field devices, e.g., a high voltage transmission relay. Ultimately, an attacker may succeed in penetrating into a computer that controls a relay, and trip the associated line. Such a line trip would cause power flow redistribution over the adjacent transmission lines and potentially lead to line overflows that induce cascading line trips. 
% kat 9/13/14 I think it's okay to just say this since we defined what this meant earlier
This could result in the system entering an emergency state.
%serious brownout voltage drop situations in load regions. 

{\bf Attack trees.} Attack trees \cite{Schneier99} and related attack graphs \cite{Lippmann05} are a useful way to capture threats against a system. An attack tree is a representation of potential attacks, with the goal of the attack at the root of the tree and the steps to achieve the attack as leaf nodes.  In this work, we use attack trees as a primary way to capture our cyber-physical threat model with respect to power system contingencies. In particular, we focus on cyber-intrusions that could lead to line contingencies. 
%Attack tree approach evolved from fault tree analysis (FTA) approach used in reliability and safety engineering.

\begin{figure*}[tb]
\centering
\includegraphics[scale=0.40]{AttackTrees-LineOutage.jpg}
\caption{High-level attack tree for line outage} 
\label{fig:tm-lineoutage}
\vspace{-0.2in}
\end{figure*}

Figure \ref{fig:tm-lineoutage} shows a high-level attack tree for line outages. This is modeled after National Electric Sector Cybersecurity Organization Resource (NESCOR) Technical Working Group 1's (TWG1) draft document\footnote{\url{http://www.smartgrid.epri.com/doc/NESCOR_10_25_12.pdf}} that presents failure scenarios for the grid with a preliminary impact analysis. As shown in the figure, line outages could be caused by, but not limited to, i) a compromised relay sending unauthorized open commands or a relay acting on compromised settings, or ii) false command injection (including changing relay settings) by a compromised operator HMI or on a compromised communication link between HMI and relay, or iii) a line open command sent by an operator who was misled by false sensor data, or iv) protection systems kicking in after other potentially maliciously induced line outages, or v) a compromised breaker. The light red color box indicates that a tree below is omitted for brevity. For example, the ``Malware'' box under ``Sensor Compromised" has the same sub-tree as the ``Malware'' box under ``Compromised Relay or Settings". 
%There are potentially many ways an adversary may gain access to a relay or cause a relay to open a line. We show a few possibilities here but are by no means exhaustive. 
The number of possibilities and actual feasible attack paths depend on the specifics of the infrastructure such as its components and its vulnerabilities.
%Similarly, false data or commands may be injected in many different ways and we highlight a few here.

{\bf Vulnerabilities.} There are several sources that provide information on currently known vulnerabilities in existing power grid control and monitoring applications. Industrial control systems cyber emergency response team (ICS-CERT) is one such source. It is a collaborative effort to share control system related security incidents and mitigation measures \cite{icscert2013}. The National Vulnerability Database that concentrates on computer vulnerabilities is another source~\cite{nvd2013}. There are several frequent and easy-to-fix vulnerabilities that appear often in cyber-physical control and monitoring devices such as hard-coded unique passwords across many identical devices~\cite{icscert2013-2}, weak passwords breakable by brute-force~\cite{icscert2013-3}, and traditional buffer-overflows~\cite{icscert2013-1} since most such firmware are coded using loosely-typed programming languages.

{\bf Scalability.} In a large infrastructure there are likely to be a large number of known vulnerabilities. However, it is important to account for vulnerabilities that are actually exploitable and focus only on those attacks paths that can emerge from such exploitation. While it may not be hard to manually come up with attack avenues at a high-level, exploring these avenues at any depth could be a intensive manual effort. An automated way of generating attack trees or graphs for a given infrastructure based on high-level attack tree templates that are created manually would be ideal and would be a good topic for future work. Right now this has to be done manually. One way to keep this tractable is to aggregate multiple vulnerabilities into a probability value indicating how easy or hard it is to transition from one node in the topology representing the infrastructure to another node along an attack path. Probability values can be computed based on the ``difficulty" (of exploiting) rating that is included in ICS-CERT advisories. For example, an easy to exploit vulnerability may be translated to a high transition probability value (say 0.75), where as a hard to exploit vulnerability may be translated to a low transition probability value (say 0.25). Limiting the scope of the threat model to line outages also helps reduce the complexity.

{\bf Industry effort.} It is encouraging to note that North American  Electric Reliability Corporation's (NERC) Critical Infrastructure Protection (CIP) Working Group chartered a task force to develop, maintain, and analyze attack trees for the electric infrastructure. This task force is looking at cyber-physical attacks. Our framework could leverage such industry developed attack trees to power our analysis.  



\begin{comment}
Reference NERC attack tree stuff, explain how while we want to capture as much as we can ourselves about threats, its best if we have a way to use the treat models that other people or organizations develop, and even better if they can use them themselves and don't need us to necessarily see the inner parts of each attack tree, as sharing of information in particular attack trees may not be allowed for security reasons.  

Or, have code that can search real-world specific topology models for exact pre-specified attack trees and mark them in some way to focus on only analyzing those

Can use the threat model to help narrow down the scope of what needs to be included in the cyber model, could actually help with scalability by potentially focusing only on threats we care about


Our model must contain, at a minimum, the nodes of the attack trees we want to consider. 

Threat model - what dependencies are we considering, how do we handle dependencies

\subsection{Attak Trees}
-- point to NERC effort
\end{comment}


==> Topologies.tex <==
\section{Cyber-Physical Power Infrastructure Model}\label{sec:topology}

Cyber-physical topology models of the power infrastructure allow \name to determine the most important cyber-induced contingencies as well as perform analysis of their impact.  
While physical connections are traceable, non-physical dependencies can be much more hidden. We develop our models using object-oriented principles, allowing new information to easily be added as it is known.  

\subsection{Power System Model}
The power system model describes the configuration and electrical characteristics of the components.
The topology describes how components are connected, while the state refers to the voltage and angle values of the electric power system at a particular instance in time.  The model often represents a best guess of what the future will hold or an estimation of the current power system conditions.  In an online sense, approximately every 3-5 minutes, a state estimator fits measured data to a power system model to obtain a best guess of the current conditions~\cite{MonticelliBook}.  The state estimator model can then be used for studies to determine the impact of outages on the present system state.  This process is called real-time contingency analysis.

Figure~\ref{fig-linestatus-1} shows a full breaker-level topology diagram, as would be used in a state estimator.  Even in a simple model like the one shown in Figure~\ref{fig-linestatus-1}, multiple breakers may be involved in isolating a line from the rest of the system.  For example, since breaker a1, a2, and b1 are open, Line~A is open. 

\begin{figure}[h]
  %\centering
    \vspace{-0.1in}
  \includegraphics[width=0.5\textwidth]{lineStatus.png} %cannot have underscores in the name
  \caption{Line status determination from breaker status}
  \label{fig-linestatus-1}
  \vspace{-0.1in}
\end{figure}

Measurements from the SCADA system map to devices in the full topology model.  PowerWorld implements a feature called integrated topology processing (ITP) \cite{GrijalvaITP} for the purpose of working with full topology models.  ITP performs model consolidation only internally as needed
%during the power flow solution process
to prevent numerical instability.  
%Full topology models may be generated from an energy management system (EMS). 
Most EMS systems have a feature to export the full topology model data in a text file format, which can be easily interpreted. 

%\textbf{Add table and/or figure showing an example of these connections for the 9-substation model and describe them}

%% kate 5/5/14 talk about labels to link to unique transmission system objects
%% Show an example of one of these items in a graphml format
%% look for a q3 picture?? or make simplified table


% kate 5/2/14 Pull in a lot more here (since this is one of the main things we've worked on for the last 4 quarters).  We already have this in other places - topology document(s)
\vspace{-0.1in}
\subsection{Cyber System Model}

The cyber system model describes the connectivity and interactions among cyber nodes, as well as existing security mechanisms that can restrict communication between connected hosts. Routers and firewalls determine which hosts on a network are able to communicate, and the cyber system model must represent this logical level.  
Building and managing cyber network models is a challenging process for an organization.  Automated tools can help; the \name framework makes use of Network Perception’s NP-View software \cite{NPView}, which builds a logical network model by parsing firewall rule-sets.
  
Figure \ref{fig:view}  shows side-by-side views of a sample cyber-physical model in both NP-View \cite{NPView} (left) and PowerWorld Simulator (right) \cite{simulator2005powerworld}.  The cyber topology shown captures the connections to the substation RTUs allowed by the firewall rules, but it does not capture details in the protection schemes at the substation level.  
%A more detailed version of this model is described in \cite{SGC2014}. 

%% kate 5/6/14

\begin{figure*}[htp]
  \centering
  \subfigure[Cyber Control Network]{\includegraphics[width=0.45\textwidth]{netapt}\label{fig:arch}}\hspace{0.2in}
  \subfigure[Power System]{\includegraphics[width=0.45\textwidth]{PhysicalLayer}\label{fig:circuit}}\hspace{0.2in}
  \vspace{-0.1in}
  \caption{Side-by-side views of a sample cyber-physical model as seen in NP-View and in PowerWorld Simulator}
  \vspace{-0.1in}
  \label{fig:view}
\end{figure*}


%%%% kate 5/5/14 CPTL %%%
There is currently no universal format to exchange cyber topologies, yet it is necessary for the future of cyber-physical modeling that we can easily store and accept information in a well-defined, easy to handle format. The CPTL language \cite{weaverChehSEGS} being developed at the University of Illinois is our candidate for developing models for this framework.  CPTL explicitly captures the cyber model information and its connections with the power model.  These cyber-physical interconnections are critical to the analysis.

%-- object oriented
